Non-Parametric Estimation of Manifolds from Noisy Data

A common observation in data-driven applications is that high dimensional data has a low intrinsic dimension, at least locally. In this work, we consider the problem of estimating a $d$ dimensional sub-manifold of $\mathbb{R}^D$ from a finite set of noisy samples. Assuming that the data was sampled uniformly from a tubular neighborhood of $\mathcal{M}\in \mathcal{C}^k$, a compact manifold without boundary, we present an algorithm that takes a point $r$ from the tubular neighborhood and outputs $\hat p_n\in \mathbb{R}^D$, and $\widehat{T_{\hat p_n}\mathcal{M}}$ an element in the Grassmanian $Gr(d, D)$. We prove that as the number of samples $n\to\infty$ the point $\hat p_n$ converges to $p\in \mathcal{M}$ and $\widehat{T_{\hat p_n}\mathcal{M}}$ converges to $T_p\mathcal{M}$ (the tangent space at that point) with high probability. Furthermore, we show that the estimation yields asymptotic rates of convergence of $n^{-\frac{k}{2k + d}}$ for the point estimation and $n^{-\frac{k-1}{2k + d}}$ for the estimation of the tangent space. These rates are known to be optimal for the case of function estimation.

==> Section_ProofStep2_BoundTf_Tf_tilde_old.tex <==
In this subsection we prove the following lemma.
\begin{Lemma}\label{lem:Tf_TtildeF}
    Let $0<\alpha_\ell = \maxangle (H_{\ell}, T f_\ell)$ be sufficiently small.
    Then, under the assumptions of Theorem \ref{thm:Step2} we have
    \[
	0 < \maxangle(T f_\ell, T {\wtilde{f}_\ell}) \leq  1/5 \tan \alpha_\ell.
	\]
\end{Lemma}
For convenience, and without limiting the generality, we assume throughout this subsection that the origin of the coordinates is a point on the manifold (i.e., $f_\ell(0)=0$ and $q_{\barak{\ell}} = 0$). 
Furthermore, in the beginning of our discussion we add the assumption that $D=d+1$ (i.e., $\MM$ is of co-dimension 1). 
This assumption will be dropped near the end of this section, once we generalize the result for arbitrary co-dimension.

As noted above, the samples of $f_\ell$ are given from a conditioned distribution $\eta_\ell(y, x)$ for $x\in H_\ell$ restricted to some neighborhood of $0$.
Furthermore, $\eta_\ell$ is supported on the finite interval $[\eta^{\min}_\ell(x), \eta^{\max}_\ell(x)]$.
Since $D=d+1$ (i.e., the $\eta_\ell(y |x)$ is scalar valued) we can denote
\[
l_{max}(x) = (x, \eta^{\max}_\ell(x))\in \RR^D
,\]
and
\[
l_{min}(x) = (x, \eta^{\min}_\ell(x))\in \RR^D
\]
Thus, we obtain
\begin{equation}\label{eq:fTilde_avg}
\wtilde{f}_\ell(x) = \frac{\eta^{\max}_\ell(x) + \eta^{\min}_\ell(x)}{2}    
.\end{equation}

Since $l_{max}(x)\in\MM_\sigma$, there exists  $\wtilde{x}(x)\in H_\ell$ such that
\[
\norm{(\wtilde x(x), f_\ell(\wtilde x(x)) - l_{max}(x)} = \sigma
.\]
That is $\wtilde{x}$ is a function from $H_\ell$ to $H_\ell$, and
\begin{equation} \label{eq:l_max_def_clean}
(\wtilde{x}(x), f_\ell(\wtilde x(x))) + \sigma \cdot \vec N = l_{max}(x),    
\end{equation}
where $\vec N(f_\ell(\wtilde x(x)))$ is the normal to the graph of the function $f_\ell$ at the point $\wtilde x(x)$.
Notice, that there exists only one such $\wtilde{x}(x)$ for every $x\in H_\ell$ as we are in the reach neighborhood.

In essence, bounding the difference between the tangents $T f_\ell, T f_\ell\in Gr(d, D)$ is the same as bounding the difference between the gradients of $f_\ell$ and $\wtilde{f}_\ell$.
Using \eqref{eq:fTilde_avg}, we arrive at
\begin{align}\label{eq:nabla_f_tilde_diff_by_l_max_clean}
\begin{split}
    \norm{ \nabla f_\ell(0) -\nabla\wtilde{f}_\ell(0)} &= \norm{ \nabla f_\ell(0) -\frac{\nabla \eta^{\max}_\ell(0) + \nabla \eta^{\min}_\ell(0)}{2}}\\\\
    &\leq 
    \frac{1}{2}\norm{ \nabla f_\ell(0) -\nabla \eta^{\max}_\ell(0)} + \frac{1}{2}\norm{ \nabla f_\ell(0) - \nabla \eta^{\min}_\ell(0)}.    
\end{split}
\end{align}
Note that, from \eqref{eq:l_max_def_clean} and from the fact that $N(f(x)) = \frac{(-\nabla f(x),1)}{\sqrt{\|\nabla_{{x}} f({x})\|^2+1}} $ we have, 
\[
\eta^{\max}_\ell(x) = f_\ell(\wtilde{x}) + \sigma \frac{1}{\sqrt{\|\nabla_{\wtilde{x}} f_\ell(\wtilde{x})\|^2+1}}
,\]
where $\nabla_{\wtilde x} $ is the gradient with respect to the composite variable $\wtilde x$.
If we denote by $J_{\wtilde x}$ the Jacobian matrix of $\wtilde x(x)$, then by the chain rule we obtain
\[
\nabla_x f_\ell(\wtilde{x}) = J_{\wtilde{x}}^T \nabla_{\wtilde{x}} f_\ell(\wtilde{x})
,\]
and as a result we have,
\[
\nabla \eta^{\max}_\ell(x) = J_{\wtilde{x}}^T \nabla_{\wtilde{x}} f_\ell(\wtilde{x}) -  
\sigma \frac{J_{\wtilde{x}}^T \HH_{\wtilde{x}}(f_\ell(\wtilde{x}))  \nabla_{\wtilde{x}} f_\ell(\wtilde{x})}{(\|\nabla_{\wtilde{x}} f_\ell(\wtilde{x})\|^2+1)^{3/2}}
,\]
where $\HH_{\wtilde{x}}(f_\ell(\wtilde x))$ denotes the Hessian of $f_\ell$ with respect to the composite variable $\wtilde x$.
Rewriting this expression we get
\begin{equation}\label{}
\nabla \eta^{\max}_\ell(x) = J_{\wtilde{x}}^T\left(I_d -  \sigma \frac{\HH_{\wtilde{x}}(f_\ell(\wtilde{x}))}{(\|\nabla_{\wtilde{x}} f_\ell(\wtilde{x})\|^2+1)^{3/2}}\right) \nabla_{\wtilde{x}} f_\ell(\wtilde{x}).
\end{equation}
Thus, in order to bound  $\nabla \eta^{\max}_\ell(0)$ and its difference from $\nabla f_\ell(0)$, we need to bound this expression evaluated at zero. 
As a preliminary step we bound the behavior of $\wtilde{x}(0)$.
\begin{Lemma}\label{lem:wtilde_x_bound_clean}
	In the aforementioned setting, we have
	\begin{equation}\label{eq:wtilde_x_bound_clean}
	0 \leq \|\wtilde{x}(0)\| \leq \sigma \sin 4\alpha_\ell
	\end{equation}
	\mycomment{I do not like this formulation, I think there should be more information in the formulation of the lemma, let's discuss how to write it}
\end{Lemma}
\begin{proof}
	Let us denote by $\alpha$, the angle
	\[
	\alpha \defeq\maxangle(T f_\ell, T f_\ell(\wtilde x(0)))
	,\]
	where $T f_\ell(\wtilde x(0))$ is the tangent space to $f_\ell$, and without limiting the generality assume that $\alpha>0$.
	Then, since 
	\[
	\norm{(\wtilde x(x), f_\ell(\wtilde x(x)) - l_{\max}} = \sigma
	,\]
	we get
	\begin{equation}\label{eq:xtilde_alpha_bound}
	\norm{\wtilde{x}(0)} \leq \sigma \sin \alpha    
	\end{equation}
	(see Figure \ref{fig:draw_step_2_bias_clean}).
	
	Using the triangle inequality for maximal angles we have that 
	\[
	\maxangle(T f_\ell, H_\ell) \leq \maxangle(T f_\ell,T f_\ell(\wtilde{x}(0))+\maxangle(T f_\ell(\wtilde{x}(0)),H_\ell),\]
	which can be written as 
	\[\alpha_\ell - \alpha \leq \maxangle(T f_\ell(\wtilde{x}(0)),H_\ell)
	,\]
	and so we achieve \barak{[shouldn't we say something about the sign of $\alpha_\ell - \alpha$? we can assume that $\alpha > 0$ and that the RHS as well is positive.]}
	\[
	\sin(|\alpha_\ell - \alpha|/2) \leq \sin(\maxangle(T f_\ell(\wtilde{x}(0)),H_\ell)/2)
	.\]
	Combining this with corollary 12 (or 3.6 \barak{[We should choose which]}) in \cite{boissonnat2017reach} we have
	\begin{equation}\label{eq:sin_alpha_1}
	\sin(|\alpha - \alpha_\ell|/2) \leq \frac{\sqrt{\norm{\wtilde{x}(0)}^2 + f_\ell(\wtilde{x}(0))^2}}{2\tau}
	\end{equation}
	From the bound on the reach, recalling the assumption that $f_\ell(0) = 0$, as well as Lemma \ref{lem:f_bound_circle_clean}, we have that for any $x$ near $0$
	\begin{equation}\label{eq:circleBound_fl}
	|f_\ell(x)| \leq \tau \cos \alpha_\ell - \sqrt{\tau^2-(\norm{x}+\tau \sin \alpha_\ell)^2}
	.\end{equation}
	That is, $f_\ell$ cannot grow faster then a circle of radius $\tau$. Thus,
	\begin{align*}
	\abs{f_\ell(\wtilde{x}(0))}^2 &\leq  (\tau \cos \alpha_\ell - \sqrt{\tau^2-(\norm{\wtilde x(0)}+\tau \sin \alpha_\ell)^2})^2 \\
	& = \tau^2 \cos^2({\alpha_\ell}) - 2\tau \cos\alpha_\ell\sqrt{\tau^2-(\norm{\wtilde x(0)}+\tau \sin \alpha_\ell)^2} + \tau^2 - (\norm{\wtilde x(0)}+\tau \sin \alpha_\ell)^2\\
	& = (1 + cos(2\alpha_\ell)) \tau^2 - \norm{\wtilde x(0)}^2 - 2\tau(\sin\alpha_\ell\norm{\wtilde x(0)} + \cos\alpha_\ell\sqrt{\tau^2-(\norm{\wtilde x(0)}+\tau \sin \alpha_\ell)^2})
	.\end{align*}
	Plugging this to \eqref{eq:sin_alpha_1} we get
	
	\begin{align*}
	    \sin(\frac{|\alpha - \alpha_\ell|}{2}) & \leq \frac{\sqrt{\tau^2 + \tau^2 \cos(2\alpha_\ell) - 2\tau \norm{\wtilde{x}} \sin\alpha_\ell- 2\tau \cos \alpha_\ell \sqrt{\tau^2 - \left(\norm{\wtilde{x}}+\tau\sin\alpha_\ell\right)^2}}}{2\tau} \\
	    & = \frac{\sqrt{1 + \cos(2\alpha_\ell) - 2\frac{\norm{\wtilde{x}}}{\tau}  \sin\alpha_\ell- 2 \cos \alpha_\ell \sqrt{1 - \left(\frac{\norm{\wtilde{x}}}{\tau}+\sin\alpha_\ell\right)^2}}}{2}
	.\end{align*}
	Given $\alpha_\ell$ sufficiently small and applying the Taylor bound of Remark \ref{rem:taylor_sqrt1-x2_clean} this can be further simplified to
	\begin{align*}
	    \sin(\frac{|\alpha - \alpha_\ell|}{2}) & \leq
	    \frac{\sqrt{1 + \cos(2\alpha_\ell) - 2\frac{\norm{\wtilde{x}}}{\tau} \sin\alpha_\ell- 2 \cos \alpha_\ell \lrbrackets{1 - \left(\frac{\norm{\wtilde{x}}}{\tau}+\sin\alpha_\ell\right)^2}}}{2} \\
	    \sin^2(\frac{|\alpha - \alpha_\ell|}{2}) & \leq
	    \frac{{1 + \cos(2\alpha_\ell) - 2\frac{\norm{\wtilde{x}}}{\tau} \sin\alpha_\ell- 2 \cos \alpha_\ell \lrbrackets{1 - \left(\frac{\norm{\wtilde{x}}}{\tau}+\sin\alpha_\ell\right)^2}}}{4} \\
	    & =
	    \frac{{1 + \cos(2\alpha_\ell) - 2 \cos \alpha_\ell - 2\frac{\norm{\wtilde{x}}}{\tau} \sin\alpha_\ell + 2 \cos \alpha_\ell \left(\frac{\norm{\wtilde{x}}}{\tau}+\sin\alpha_\ell\right)^2}}{4}
	.\end{align*}
	Since $\alpha_\ell > 0$ we can further simplify the expression to
	\begin{align*}
	    \sin(\frac{|\alpha - \alpha_\ell|}{2}) & \leq
	    \frac{{1 + \cos(2\alpha_\ell) + 2 \cos \alpha_\ell \left(\frac{\norm{\wtilde{x}}}{\tau}+\sin\alpha_\ell\right)^2}}{4} \\
	    & = 
	    \frac{{2 - 2\cos(\alpha_\ell) + 2 \cos \alpha_\ell \left(\frac{\norm{\wtilde{x}}}{\tau}+\sin\alpha_\ell\right)^2}}{4} \\
	    & = 
	    \frac{{1 - \cos(\alpha_\ell) +  \cos \alpha_\ell \left(\frac{\norm{\wtilde{x}}}{\tau}+\sin\alpha_\ell\right)^2}}{2}
	.\end{align*}
	Plugging in \eqref{eq:xtilde_alpha_bound} we get
	\begin{align}\label{eq:sin_alpha-alpha_0_square_clean}
	    \sin(\frac{|\alpha - \alpha_\ell|}{2}) & \leq
	    \frac{{1 - \cos(\alpha_\ell) +  \cos \alpha_\ell \left(\frac{\sigma}{\tau}\sin\alpha+\sin\alpha_\ell\right)^2}}{2}
	\end{align}
	\iffalse
	$$
	\begin{array}{ll}
	\sin(\frac{|\alpha - \alpha_0|}{2}) & \leq
	\frac{\sqrt{\norm{\wtilde{x}(0)}^2 + f_\ell(\wtilde{x}(0))^2}}{2\tau} \\
	& = \frac{1}{2\tau}\sqrt{\norm{\wtilde{x}}^2+\tau^2 \cos^2\alpha_0 +(\tau^2 - (\norm{\wtilde{x}}+\tau\sin\alpha_0)^2) - 2\tau \cos \alpha_0 \sqrt{\tau^2 - (\norm{\wtilde{x}}+\tau\sin\alpha_0)^2}} \\
	& = \frac{1}{2\tau}\sqrt{\tau^2 + \tau^2 \cos(2\alpha_0) - 2\tau \norm{\wtilde{x}} \sin\alpha_0- 2\tau \cos \alpha_0 \sqrt{\tau^2 - \left(\norm{\wtilde{x}}+\tau\sin\alpha_0\right)^2}}\\
	& \leq \frac{1}{2}\sqrt{1 + \cos(2\alpha_0) - 2 \frac{\norm{\wtilde{x}}}{\tau} \sin\alpha_0- 2 \cos \alpha_0 \left(1 - 2/3 \left(\frac{\norm{\wtilde{x}}}{\tau}+\sin\alpha_0\right)^2\right)}
	\end{array}
	$$
	or, 
	\begin{equation}\label{eq:sin_alpha-alpha_0_square_clean}
	\begin{array}{ll}
	\sin^2(\frac{\alpha-\alpha_0}{2}) & \leq \frac{1}{4}\left( 1 + \cos(2\alpha_0) - 2 \frac{\norm{\wtilde{x}}}{\tau} \sin\alpha_0- 2 \cos \alpha_0 \left(1 - 2/3 \left(\frac{\norm{\wtilde{x}}}{\tau}+\sin\alpha_0\right)^2\right)\right)\\
	&=\frac{1}{4}\left( 1 + \cos(2\alpha_0) - 2\cos \alpha_0 + \frac{4}{3} \cos \alpha_0 \left(\frac{\norm{\wtilde{x}}}{\tau}+\sin\alpha_0\right)^2 - 2 \frac{\norm{\wtilde{x}}}{\tau} \sin\alpha_0\right)\\
	& \leq \frac{1}{4}\left( 2 - 2 \cos\alpha_0 + \frac{4}{3} \left(\sin\alpha_0+ \frac{\norm{\wtilde{x}}}{\tau}\right)^2\right)\\
	& = \frac{1}{2}\left( 1 - \cos(\alpha_0) + \frac{2}{3} \left(\sin\alpha_0+ \frac{\sigma}{\tau}\sin\alpha\right)^2\right)
	\end{array}
	\end{equation}
	\fi
	Note that we expect to have no bias if $\alpha_\ell=0$ and indeed, for $\alpha_\ell = 0$ we have
	\[
	\sin^2(\frac{\alpha}{2}) \leq \frac{\sigma^2}{2\tau^2}\sin^2\alpha
	.\]
	and thus for $\tau$ large enough $\alpha_\ell = 0 \implies \alpha = 0 \implies \wtilde{x} = 0 \implies$ there is no bias.
	
	Using the following inequalities (for sufficiently small $\alpha_\ell$)
	$$
	\begin{array}{rcl}
	\frac{1}{2}\zeta^2 &\leq& \sin (\zeta)^2\\
	-\cos(\alpha_\ell)&\leq& -(1-\alpha_\ell^2/2) \\
	\sin \alpha_\ell &\leq& \alpha_\ell\\
	\sin \alpha &\leq& \alpha
	\end{array}
	$$
	we simplify \eqref{eq:sin_alpha-alpha_0_square_clean} and get
	\begin{align*}
	    \frac{(\alpha-\alpha_\ell)^2}{8} &\leq \frac{1}{2}\left( 1 - (1-\alpha_\ell^2/2) +  \left(\frac{\sigma}{\tau}\alpha + \alpha_\ell\right)^2\right) \\
	    \frac{\alpha^2-2\alpha\alpha_\ell + \alpha_\ell^2}{8} &\leq \frac{1}{2}\left( -\frac{\alpha_\ell^2}{2} + \frac{\sigma^2}{\tau^2}\alpha^2 + 2 \frac{\sigma}{\tau} \alpha \alpha_\ell + \alpha_\ell^2\right) \\ 
	    0 & \leq
	    \lrbrackets{\frac{\sigma^2}{\tau^2} - \frac{1}{8}}\alpha^2 + \lrbrackets{\frac{1}{2} - \frac{1}{8}}\alpha_\ell^2 + \lrbrackets{2\frac{\sigma}{\tau} + \frac{1}{4}}\alpha \alpha_\ell \\
	    0 & \leq
	    \lrbrackets{\frac{\sigma^2}{\tau^2} - \frac{1}{8}}\alpha^2 + { \frac{3}{8}}\alpha_\ell^2 + \lrbrackets{2\frac{\sigma}{\tau} + \frac{1}{4}}\alpha \alpha_\ell 
	.\end{align*}
	The right hand side of this expression is a parabola with respect to $\alpha$.
	For $\frac{\sigma}{\tau} = 0$ the roots are $\alpha = -{\alpha_\ell}, {3\alpha_\ell}$.
	Thus, from continuity of the roots, for sufficiently small $\frac{\sigma}{\tau}$ we get $\alpha \leq 4 \alpha_\ell$.
	For example, by setting $\frac{\sigma}{\tau} = 0.09$ the claim is already true.
	Thus, since we know from \eqref{eq:xtilde_alpha_bound} that $\norm{\wtilde{x}(0)}\leq \sigma \sin\alpha$ we get
	\[
	0 \leq \norm{\wtilde x(0)} \leq \sigma \sin 4 \alpha_\ell
	,\]
	as required.
	\iffalse
	\begin{equation} \label{eq:square_eq_on_alpha_clean}
	\begin{array}{rl}
	\frac{1}{2}(\frac{\alpha-\alpha_0}{2})^2 &\leq \frac{1}{2}\left( 1 - (1-\alpha_0^2/2) + \frac{2}{3} \left(\alpha_0+ \frac{\sigma}{\tau}\alpha\right)^2\right)\\
	1/8(\alpha^2+\alpha_0^2 - 2\alpha \alpha_0)& \leq \frac{1}{2}\left( \alpha_0^2/2 + \frac{2}{3} \alpha_0^2+ \frac{2\sigma^2}{3\tau^2}\alpha^2 + \frac{4}{3}\alpha_0 \frac{\sigma}{\tau}\alpha  \right) \\
	0& \leq \left(\frac{\sigma^2}{3\tau^2}-1/8\right)\alpha^2 + \left(\frac{1}{3} + \frac{1}{8}\right) \alpha_0^2+ \left(\frac{2\sigma}{3\tau} + \frac{1}{4}\right)\alpha_0 \alpha.
	\end{array}
	\end{equation}
	The right hand side of Eq.~\eqref{eq:square_eq_on_alpha_clean} gives us a parabola. For $\sigma/\tau = 0$ the roots are $\alpha = \alpha_0(1 \pm \sqrt{\frac{14}{3}})$.
	%(using $\sin x = x$ will result in $\alpha = \alpha_0(1 \pm \sqrt{\frac{7}{3}})$)
	% , since
	% \[
	% \alpha_{1,2} = \frac{-\frac{1}{4}\alpha_0 \pm \sqrt{\frac{1}{16}\alpha_0^2+4\frac{1}{8}\left(\frac{1}{3} + \frac{1}{8}\right)\alpha_0^2}}{-\frac{1}{4}}
	% \]
	For $\sigma/\tau < 0.1$, we have, due to continuity, that 
	$ \alpha \leq 4\alpha_0 = \alpha_{max}$. 
	Thus, since $\|\wtilde{x}(0)\| = \sigma \sin \alpha$, we have
	\begin{equation} 
	0 \leq \|\wtilde{x}(0)\| \leq \sigma \sin 4\alpha_0
	\end{equation}
	\fi
\end{proof}
Before bounding the Jacobi matrix of $\wtilde{x}$ we will show the following lemma
\begin{Lemma}\label{lem:gradient_and_hessian_bounds_clean}
	For  $\alpha_\ell \leq \pi/4$, and some constant $c_1$, 
	\begin{equation}\label{eq:nabla_f_bound_clean}
	\| \nabla_{\wtilde{x}}f(\wtilde{x})\|^2 \leq 
	d \tan^2 \alpha_0\left(1 +c_1  \frac{\sigma}{\tau}\right)^2,    
	\end{equation}
	
	\begin{equation}\label{eq:nabla_f_diff_bound_clean}
	\|\nabla_{\wtilde{x}} f(\wtilde{x}) -\nabla f(0) \|^2 \leq d\tan^2 \alpha_0 \left(c_1\frac{\sigma}{\tau}\right)^2,    
	\end{equation}
	
	\begin{equation}\label{eq:nabla_f_nabla_fT_bound_clean}
	\left\| \nabla_{\wtilde{x}} f(\wtilde{x})
	\nabla_{\wtilde{x}} f(\wtilde{x})^T \right\|_{op} 
	\leq d \tan^2 \alpha_0\left(1 +c_1  \frac{\sigma}{\tau}\right)^2,  
	\end{equation}
	and
	\begin{equation}\label{eq:hessian_bound_clean}
	\left\|\frac{\HH_{\wtilde{x}}}{\left(\|\nabla_{\wtilde{x}} f(\wtilde{x})\|^2+1\right)^{3/2}}\right\|_{op} \leq \frac{1}{\tau}    
	\end{equation}
	where $\HH_{\wtilde{x}}$ is the Hessian of $f$ at $\wtilde{x}$.
\end{Lemma}

\begin{proof}
	First we recall the result for the 1-D case of Lemma \ref{lem:derivative_bound_1D_clean}. For a 1-dimensional function f, who's graph has a bounded reach $\tau$, and assuming $f'(0)\leq \alpha_0$ we have
	\[
	\tan \alpha_0 - \frac{x}{\tau \cos \alpha_0} \leq f'(x) \leq  \tan \alpha_0 +  \frac{x}{\tau\cos^3 \alpha_0},
	\]
	Assuming $x \leq \sigma \sin 4\alpha_0$, we have 
	\[
	\tan \alpha_0 - \frac{\sigma \sin 4\alpha_0}{\tau \cos \alpha_0} \leq f'(x) \leq  \tan \alpha_0 +  \frac{\sigma \sin 4\alpha_0}{\tau\cos^3 \alpha_0},
	\]
	Notice that for $\alpha_0 \leq \pi/4$, $\cos^2 \alpha_0$ is larger than some constant. Additionally, notice that $\sin (4\alpha_0) \leq 4 \sin(\alpha_0)$ since
	\[sin(\alpha_0) \leq \alpha_0\]
	\[ 
	4 sin(\alpha_0) \geq 4 \alpha_0 - \frac{(4 \alpha_0)^3}{3!} \geq \alpha_0 .
	\]
	Thus, we have 
	\begin{equation}\label{eq:f'_bound_small_x_clean}
	\tan \alpha_0 \left(1-c_1\frac{\sigma }{\tau }\right) \leq f'(x) \leq   \tan \alpha_0 \left(1 +  c_1\frac{\sigma }{\tau}\right),    
	\end{equation}
	for  $c_1 = 4/\cos^2 (\pi/4)$.
	
	\textbf{Proof of \eqref{eq:nabla_f_bound_clean}}: In order to bound the gradient of f at $\wtilde{x}$ we note that each coordinate of the gradient behaves the same as 1-dimensional function, thus
	\[
	\| \nabla_{\wtilde{x}}f(\wtilde{x})\|^2 \leq d \max_i f_i'(\wtilde{x})^2 \leq d \tan^2 \alpha_0 \left(1 +  c_1\frac{\sigma }{\tau}\right)^2
	\]
	
	\textbf{Proof of \eqref{eq:nabla_f_diff_bound_clean}}: Again, using Eq. \eqref{eq:f'_bound_small_x_clean}, for each coordinate seperatly, and using the fact that the angle at $0$ at any direction is bounded by $\alpha_0$ we have that 
	\[
	\|\nabla_{\wtilde{x}} f(\wtilde{x}) -\nabla f(0) \|^2 \leq d\tan^2 \alpha_0 \left(c_1\frac{\sigma}{\tau}\right)^2, 
	\]
	
	\textbf{Proof of \eqref{eq:nabla_f_nabla_fT_bound_clean}}
	We bound $\nabla_{\wtilde{x}} f(\wtilde{x})
	\nabla_{\wtilde{x}} f(\wtilde{x})^T $
	\[
	\left|\left(\nabla_{\wtilde{x}} f(\wtilde{x})
	\nabla_{\wtilde{x}} f(\wtilde{x})^T \right)_{i,j}\right| = \left|\frac{\partial f}{\partial x_i} \frac{\partial f}{\partial x_j}\right| \leq \tan^2 \alpha_0 \left(1 +  c_1\frac{\sigma }{\tau}\right)^2
	\]
	thus,
	\[
	\left\| \nabla_{\wtilde{x}} f(\wtilde{x})
	\nabla_{\wtilde{x}} f(\wtilde{x})^T \right\|_{op} 
	\leq d \tan^2 \alpha_0 \left(1 +  c_1\frac{\sigma }{\tau}\right)^2
	\]
	
	\textbf{Proof of \eqref{eq:hessian_bound_clean}}
	There is an orthogonal transformation/change of coordinates such that $H_{\wtilde{x}}$ is diagonal.
	Since $\|H_{\wtilde{x}}\| = \|U^TH_{\wtilde{x}}U\|$  we can bound the diagonal version of $H_{\wtilde{x}}$. Thus, the problem is reduced to bounding the second derivative of $d$ functions of from $\RR$ to $\RR$.
	\item Denote $\bar{x}_1, \ldots, \bar{x}_d $ the new diagonalizeing coordinate system, and denote $f_i$ to be the slice of $f$ in the direction $\bar{x}_i$ for which the second derivative is maximal. 
	Then, since H is diagonal, it's norm is equal to the maximal value ($\|H_{\wtilde{x}}\| = |f_i''(\wtilde{x})|$).
	\[
	\left\|\frac{H_{\wtilde{x}}}{\left(\|\nabla_{\wtilde{x}} f(\wtilde{x})\|^2+1\right)^{3/2}}\right\|_{op} \leq 
	\frac{|f''_i(\wtilde{x})|}{ ({f'_i}^2 + 1)^{3/2} } \leq \frac{1}{\tau}
	\]
	
\end{proof}
Next we bound the Jacobi matrix
\begin{Lemma}\label{lem:Jacobi_bound_clean}
	In the setting above, assuming $\alpha_0 \leq \pi/4$, the Jacobi matrix of $\wtilde{x}$ at $0$, $J_{\wtilde{x}}(0)$ is bounded by
	\begin{equation}
	\left\| J_{\wtilde{x}}^T\right\| \leq 1 + 2\frac{\sigma}{\tau} \left(  1 + 2
	d \tan^2 \alpha_0\left(1 +c_1  \frac{\sigma}{\tau}\right)^2 \right),
	\end{equation}
	where $c_1 = 4/\cos^2 (\pi/4)$
\end{Lemma}
\begin{proof}
	\[
	\wtilde{x} - x = \frac{\sigma \nabla f(\wtilde{x})}{ \sqrt{\|\nabla f(\wtilde{x})\|^2+1}}
	\]
	Writing $\wtilde{x}$ as an implicit function of $x$ we have 
	\[
	G(\wtilde{x},x) = \wtilde{x} - x - \frac{\sigma \nabla f(\wtilde{x})}{ \sqrt{\|\nabla f(\wtilde{x})\|^2+1}} = \vec{0}
	\]
	Using the Implicit function theorem we have the Jacobi matrix of $\wtilde{x}$
	\[
	J_{\wtilde{x}} = \frac{d\wtilde{x}}{dx} = -\left(\frac{\partial G}{\partial \wtilde{x}}\right)^{-1} \frac{\partial G}{\partial x} 
	\]
	\[
	\frac{\partial G}{\partial x} = -I
	\]
	\[
	\frac{\partial G}{\partial \wtilde{x}} = I - \sigma \frac{H_{\wtilde{x}}(f(\wtilde{x})) \sqrt{\|\nabla_{\wtilde{x}} f(\wtilde{x})\|^2+1} - \nabla_{\wtilde{x}} f(\wtilde{x}) \left(\nabla(\sqrt{\|\nabla_{\wtilde{x}} f(\wtilde{x})\|^2+1})\right)^T  }{\|\nabla_{\wtilde{x}} f(\wtilde{x})\|^2+1}
	\]
	\[
	=  I - \sigma \frac{H_{\wtilde{x}}(f(\wtilde{x})) \sqrt{\|\nabla_{\wtilde{x}} f(\wtilde{x})\|^2+1} - \nabla_{\wtilde{x}} f(\wtilde{x})
		\frac{1}{2\sqrt{\|\nabla_{\wtilde{x}} f(\wtilde{x})\|^2+1}}
		v^T  }{\|\nabla f(\wtilde{x})\|^2+1}
	\]
	Where $v = \nabla_{\wtilde{x}} (\|\nabla_{\wtilde{x}} f(\wtilde{x})\|^2) = \nabla_{\wtilde{x}} (\nabla_{\wtilde{x}} f(\wtilde{x})^T \nabla f(\wtilde{x}))$
	\[
	\nabla_{\wtilde{x}} f(\wtilde{x})^T \nabla_{\wtilde{x}} f(\wtilde{x}) = \sum \left(\frac{\partial f}{\partial \wtilde{x}_i}\right)  ^2
	\]
	\[
	\frac{\partial (\nabla_{\wtilde{x}} f(\wtilde{x})^T \nabla_{\wtilde{x}} f(\wtilde{x}))}{\partial x_j} = \sum_i 2\frac{\partial f}{\partial \wtilde{x}_i} \frac{\partial^2 f}{\partial \wtilde{x}_i \partial \wtilde{x}_j}   
	\]
	Then $v = 2H_{\wtilde{x}}(f(\wtilde{x})) \nabla_{\wtilde{x}} f(\wtilde{x})$
	\[
	=  I - \sigma \frac{H_{\wtilde{x}}(f(\wtilde{x})) \left(\|\nabla_{\wtilde{x}} f(\wtilde{x})\|^2+1\right) - \nabla_{\wtilde{x}} f(\wtilde{x})
		\left(H_{\wtilde{x}}(f(\wtilde{x})) \nabla_{\wtilde{x}} f(\wtilde{x})\right)^T  }{\left(\|\nabla_{\wtilde{x}} f(\wtilde{x})\|^2+1\right)^{3/2}}
	\]
	\[
	=  I - \sigma \frac{H_{\wtilde{x}}(f(\wtilde{x})) \left(\|\nabla_{\wtilde{x}} f(\wtilde{x})\|^2+1\right) - \nabla_{\wtilde{x}} f(\wtilde{x})
		\nabla_{\wtilde{x}} f(\wtilde{x})^T H_{\wtilde{x}}(f(\wtilde{x}))  }{\left(\|\nabla_{\wtilde{x}} f(\wtilde{x})\|^2+1\right)^{3/2}}
	\]
	Thus
	\begin{equation}\label{eq:J_equals_clean}
	J_{\wtilde{x}} = \frac{d\wtilde{x}}{dx} =  
	\left( I - \sigma \frac{H_{\wtilde{x}}(f(\wtilde{x})) \left(\|\nabla_{\wtilde{x}} f(\wtilde{x})\|^2+1\right) - \nabla_{\wtilde{x}} f(\wtilde{x})
		\nabla_{\wtilde{x}} f(\wtilde{x})^T H_{\wtilde{x}}(f(\wtilde{x}))  }{\left(\|\nabla_{\wtilde{x}} f(\wtilde{x})\|^2+1\right)^{3/2}} \right)^{-1}    
	\end{equation}
	
	
	Note that  for $A$ with $\|A\| \leq 1$
	\[
	\|(I-A)^{-1}\| = (1-\|A\|)^{-1}
	\]
	Since 
	\[ 
	\sigma \left\| \frac{H_{\wtilde{x}}(f(\wtilde{x})) \left(\|\nabla_{\wtilde{x}} f(\wtilde{x})\|^2+1\right) - \nabla_{\wtilde{x}} f(\wtilde{x})
		\nabla_{\wtilde{x}} f(\wtilde{x})^T H_{\wtilde{x}}(f(\wtilde{x}))  }{\left(\|\nabla_{\wtilde{x}} f(\wtilde{x})\|^2+1\right)^{3/2}} \right\|\leq 1
	\]
	we have that 
	\[
	\left\| J_{\wtilde{x}}^T\right\| = \left(1- \sigma \left\| \frac{H_{\wtilde{x}}(f(\wtilde{x})) \left(\|\nabla_{\wtilde{x}} f(\wtilde{x})\|^2+1\right) - \nabla_{\wtilde{x}} f(\wtilde{x})
		\nabla_{\wtilde{x}} f(\wtilde{x})^T H_{\wtilde{x}}(f(\wtilde{x}))  }{\left(\|\nabla_{\wtilde{x}} f(\wtilde{x})\|^2+1\right)^{3/2}} \right\| \right)^{-1} 
	\]
	
	and by Lemma \ref{lem:gradient_and_hessian_bounds_clean} we have:
	\begin{multline}
	\sigma \left\| \frac{H_{\wtilde{x}}(f(\wtilde{x})) \left(\|\nabla_{\wtilde{x}} f(\wtilde{x})\|^2+1\right) - \nabla_{\wtilde{x}} f(\wtilde{x})
		\nabla_{\wtilde{x}} f(\wtilde{x})^T H_{\wtilde{x}}(f(\wtilde{x}))  }{\left(\|\nabla_{\wtilde{x}} f(\wtilde{x})\|^2+1\right)^{3/2}} \right\| \\
	\leq \frac{\sigma}{\tau} \left(  
	\| \nabla_{\wtilde{x}}f(\wtilde{x})\|^2 + 1
	+  \left\| \nabla_{\wtilde{x}} f(\wtilde{x})
	\nabla_{\wtilde{x}} f(\wtilde{x})^T \right\|_{op}
	\right)  \\
	\leq  \frac{\sigma}{\tau} \left(  1 + 
	d \tan^2 \alpha_0\left(1 +c_1  \frac{\sigma}{\tau}\right)^2 
	+ d \tan^2 \alpha_0\left(1 +c_1  \frac{\sigma}{\tau}\right)^2
	\right)      \\
	\leq  \frac{\sigma}{\tau} \left(  1 + 2
	d \tan^2 \alpha_0\left(1 +c_1  \frac{\sigma}{\tau}\right)^2 \right)  
	\end{multline}
	
	
	Thus (using Taylor bound for $1/(1-x)$)
	\[
	\left\| J_{\wtilde{x}}^T\right\| \leq 1 + 2\frac{\sigma}{\tau} \left(  1 + 2
	d \tan^2 \alpha_0\left(1 +c_1  \frac{\sigma}{\tau}\right)^2 \right)
	\]  
\end{proof}

Going back to Eq. \eqref{eq:nabla_f_tilde_diff_by_l_max_clean}, and bounding $\| \nabla f(0) -\nabla l_{max}\|$
\begin{multline}\label{eq:nabla_l-nabla_f_clean}
\|\nabla l_{max} - \nabla f(0)\|  \\ 
=
\left\| J_{\wtilde{x}}^T\left(I_d -  \sigma \frac{H_{\wtilde{x}}(f(\wtilde{x}))}{(\|\nabla_{\wtilde{x}} f(\wtilde{x})\|^2+1)^{3/2}}\right) \nabla_{\wtilde{x}} f(\wtilde{x})  -  \nabla_{\wtilde{x}} f(\wtilde{x}) +\nabla_{\wtilde{x}} f(\wtilde{x}) -\nabla f(0) \right\|  \\
\leq
\left\| J_{\wtilde{x}}^T\left(I_d -  \sigma \frac{H_{\wtilde{x}}(f(\wtilde{x}))}{(\|\nabla_{\wtilde{x}} f(\wtilde{x})\|^2+1)^{3/2}}\right) \nabla_{\wtilde{x}} f(\wtilde{x})  -  \nabla_{\wtilde{x}} f(\wtilde{x}) \right\|+ \|\nabla_{\wtilde{x}} f(\wtilde{x}) -\nabla f(0) \| \\
\leq
\left\| J_{\wtilde{x}}^T\left(I_d -  \sigma \frac{H_{\wtilde{x}}(f(\wtilde{x}))}{(\|\nabla_{\wtilde{x}} f(\wtilde{x})\|^2+1)^{3/2}}\right) - I_d \right\|_{op} \|\nabla_{\wtilde{x}} f(\wtilde{x})  \|_2  + \|\nabla_{\wtilde{x}} f(\wtilde{x}) -\nabla f(0) \|_2
\end{multline}

Now, consider the left most part of Eq. \eqref{eq:nabla_l-nabla_f_clean}
\begin{multline}\label{eq:nabla_l-nabla_f_part1_clean}
\left\| J_{\wtilde{x}}^T\left(I_d -  \sigma \frac{H_{\wtilde{x}}(f(\wtilde{x}))}{(\|\nabla_{\wtilde{x}} f(\wtilde{x})\|^2+1)^{3/2}}\right) - I_d \right\|_{op} \\ 
=
\left\| J_{\wtilde{x}}^T\left(I_d -  \sigma \frac{H_{\wtilde{x}}(f(\wtilde{x}))}{(\|\nabla_{\wtilde{x}} f(\wtilde{x})\|^2+1)^{3/2}} - {J^T}^{-1}\right) \right\|_{op} \\
\leq
\left\| J_{\wtilde{x}}^T\right\|_{op} \left\|\left(I_d -  \sigma \frac{H_{\wtilde{x}}(f(\wtilde{x}))}{(\|\nabla_{\wtilde{x}} f(\wtilde{x})\|^2+1)^{3/2}} - {J^T}^{-1}\right) \right\|_{op}.
\end{multline}
Expanding the Right part of Eq. \eqref{eq:nabla_l-nabla_f_part1_clean} using \eqref{eq:J_equals_clean} and Lemma \ref{lem:gradient_and_hessian_bounds_clean}, we have 
\begin{multline}
\left\| \left(I_d -  \sigma \frac{H_{\wtilde{x}}(f(\wtilde{x}))}{(\|\nabla_{\wtilde{x}} f(\wtilde{x})\|^2+1)^{3/2}} - {J^T}^{-1}\right) \right\|_{op} =
\left\|I_d -  \sigma \frac{H_{\wtilde{x}}(f(\wtilde{x}))}{(\|\nabla_{\wtilde{x}} f(\wtilde{x})\|^2+1)^{3/2}} \right.\\ 
\left. - I_d + \sigma \frac{H_{\wtilde{x}}(f(\wtilde{x})) \left(\|\nabla_{\wtilde{x}} f(\wtilde{x})\|^2+1\right) -  H_{\wtilde{x}}(f(\wtilde{x})) \nabla_{\wtilde{x}} f(\wtilde{x})
	\nabla_{\wtilde{x}} f(\wtilde{x})^T  }{\left(\|\nabla_{\wtilde{x}} f(\wtilde{x})\|^2+1\right)^{3/2}}\right\| \\
=\left\|
\sigma \frac{H_{\wtilde{x}}(f(\wtilde{x})) \left(\|\nabla_{\wtilde{x}} f(\wtilde{x})\|^2+1\right) -  H_{\wtilde{x}}(f(\wtilde{x})) \nabla_{\wtilde{x}} f(\wtilde{x})
	\nabla_{\wtilde{x}} f(\wtilde{x})^T  - H_{\wtilde{x}}(f(\wtilde{x})) }{\left(\|\nabla_{\wtilde{x}} f(\wtilde{x})\|^2+1\right)^{3/2}} \right\|\\
=
\sigma\left\| \frac{H_{\wtilde{x}}(f(\wtilde{x})) } {\left(\|\nabla_{\wtilde{x}} f(\wtilde{x})\|^2+1\right)^{3/2}} \left( \|\nabla_{\wtilde{x}} f(\wtilde{x})\|^2  - \nabla_{\wtilde{x}} f(\wtilde{x})
\nabla_{\wtilde{x}} f(\wtilde{x})^T \right) \right\| \\
\leq 
\sigma\left\| \frac{H_{\wtilde{x}}(f(\wtilde{x})) } {\left(\|\nabla_{\wtilde{x}} f(\wtilde{x})\|^2+1\right)^{3/2}}\right\| \left\| \|\nabla_{\wtilde{x}} f(\wtilde{x})\|^2 I  - \nabla_{\wtilde{x}} f(\wtilde{x})
\nabla_{\wtilde{x}} f(\wtilde{x})^T \right\| \\
\leq
\frac{\sigma}{\tau} (  \|\nabla_{\wtilde{x}} f(\wtilde{x})\|^2 +\left\| \nabla_{\wtilde{x}} f(\wtilde{x}) 
\nabla_{\wtilde{x}} f(\wtilde{x})^T \right\| ) \\
\leq
\frac{\sigma}{\tau} (  d \tan^2 \alpha_0\left(1 +c_1  \frac{\sigma}{\tau}\right)^2 + d \tan^2 \alpha_0\left(1 +c_1  \frac{\sigma}{\tau}\right)^2) \\
\leq
2\frac{\sigma}{\tau}  d \tan^2 \alpha_0\left(1 +c_1  \frac{\sigma}{\tau}\right)^2.
\end{multline}
Substituting back into Eq.~\eqref{eq:nabla_l-nabla_f_part1_clean}, and using Lemma~\ref{lem:Jacobi_bound_clean} we have,
\begin{multline}
\left\| J_{\wtilde{x}}^T\left(I_d -  \sigma \frac{H_{\wtilde{x}}(f(\wtilde{x}))}{(\|\nabla_{\wtilde{x}} f(\wtilde{x})\|^2+1)^{3/2}}\right) - I_d \right\|_{op} \\ 
\leq
\left\| J_{\wtilde{x}}^T\right\|_{op} 2\frac{\sigma}{\tau}  d \tan^2 \alpha_0\left(1 +c_1  \frac{\sigma}{\tau}\right)^2\\
\leq
\left( 1 + 2\frac{\sigma}{\tau} \left(  1 + 2
d \tan^2 \alpha_0\left(1 +c_1  \frac{\sigma}{\tau}\right)^2 \right)\right) 2\frac{\sigma}{\tau} d \tan^2 \alpha_0\left(1 +c_1  \frac{\sigma}{\tau}\right)^2\\
\end{multline}
Substituting into Eq. \eqref{eq:nabla_l-nabla_f_clean}, we have
\begin{multline}
\|\nabla l_{max} - \nabla f(0)\| \\
\leq \left( 1 + 2\frac{\sigma}{\tau} \left(  1 + 2
d \tan^2 \alpha_0\left(1 +c_1  \frac{\sigma}{\tau}\right)^2 \right)\right) 2\frac{\sigma}{\tau} d \tan^2 \alpha_0\left(1 +c_1  \frac{\sigma}{\tau}\right)^2 \|\nabla_{\wtilde{x}} f(\wtilde{x})  \|_2  \\
+ \|\nabla_{\wtilde{x}} f(\wtilde{x}) -\nabla f(0) \|_2 \\
\leq
2\frac{\sigma}{\tau} d \tan^2 \alpha_0 \left( 1 + 2\frac{\sigma}{\tau} \left(  1 + 2
d \tan^2 \alpha_0\left(1 +c_1  \frac{\sigma}{\tau}\right)^2 \right)\right) \left(1 +c_1  \frac{\sigma}{\tau}\right)^2 
\sqrt{d} \tan \alpha_0\left(1 +c_1  \frac{\sigma}{\tau}\right) \\
+ \sqrt{d}\tan \alpha_0 \left(c_1\frac{\sigma}{\tau}\right) \\
\end{multline}

Symmetrically, the same bound applies to $\nabla l_{min}$, and thus, we get from Eq. \eqref{eq:nabla_f_tilde_diff_by_l_max_clean} that 
\begin{multline}
\| \nabla f(0) -\nabla\wtilde{f}(0)\| \leq
\frac{\sigma}{\tau} \sqrt{d} \tan \alpha_0 \\
\left( 2d^2 \tan^2 \alpha_0 \left( 1 + 2\frac{\sigma}{\tau} \left(  1 + 2
d \tan^2 \alpha_0\left(1 +c_1  \frac{\sigma}{\tau}\right)^2 \right)\right) \left(1 +c_1  \frac{\sigma}{\tau}\right)^3
+ c_1 \right).
\end{multline}
Thus, for $\frac{\sigma}{\tau}$ small enough, we have that 
\[
\| \nabla f(0) -\nabla\wtilde{f}(0)\| \leq 1/10 \tan \alpha_0.
\]


In order to extend the above result to the case of general $D$ (to relax the requirement that $D=d+1$), use the following argument.
First, repeating the above derivation, for any projection $P:\RR^{D-d} \rightarrow \RR$, we have that 
\[
\| \nabla Pf(0) -\nabla P\wtilde{f}(0)\| \leq 1/10 \tan \alpha_0.
\]
Thus, it follows that 
\[
\| J_f(0) -J_{\wtilde{f}}(0)\|_{op} \leq 1/10 \tan \alpha_0.
\]
We also need the following lemma.
\begin{Lemma}\label{lem:Q_angle_between_flats}
    Let $L_1$ and $L_2$ be two linear subspaces of $\RR^n$. Denote $Q_{L_1,L_2}:L_1 \rightarrow L_2^\perp$ defined as
    \[
    Q_{L_1,L_2}(v) = \|v - Proj_{L_2}(v)\|.
    \]
    Then $\sin \angle_{max}(L_1,L_2) = \|Q_{L_1,L_2}\|_{op}$.
\end{Lemma}

Denote by $T_f = \{(v,(J_f(0))v )| v\in \RR^d\} \subset \RR^D$ and $T_{\wtilde{f}}= \{(v,(J_{\wtilde{f}}(0))v )| v\in \RR^d\}\subset \RR^D$ the tangent of $f$ and $\wtilde{f}$ at $0$. Then, for any vector $v\in \RR^d$,
\[
\|Q_{T_f, T_{\wtilde{f}} }(v,(J_f(0))v )\| \leq \|(v,(J_f(0))v ) - (v,(J_{\wtilde{f}}(0))v )\| \leq \|J_f(0) - J_{\wtilde{f}}(0)\| \|v\| \leq \|J_f(0) - J_{\wtilde{f}}(0)\| \|(v,(J_f(0))v)\|,
\]
and thus,
\[
\sin \angle_{max}(T_f, T_{\wtilde{f}})  = \|Q_{T_f, T_{\wtilde{f}} }\|_{op} \leq \|J_f(0) - J_{\wtilde{f}}(0)\|_{op} \leq  1/10 \tan \alpha_0,
\]
or,
\begin{equation}\label{eq:ang_bound_T_f_T_f_tilde}
    \angle_{max}(T_f, T_{\wtilde{f}}) \leq  1/5 \tan \alpha_0.
\end{equation}
% Relaxing the requirement that $D=d+1$, we can repeat the same arguments for an arbitrary $D$. In the case of arbitrary $D$ we have $f:H \rightarrow \RR^{D-d}$. We can think of the $f$ as a vector $D-d$ real valued functions $f_1,\ldots, f_{D-d}$ such that $f_i:H \rightarrow \RR$ and 
% \[
% f(x) = \left(\begin{array}{c}
% f_1(x) \\
% \vdots\\
% f_{D-d}(x)
% \end{array}\right).
% \]
% We can repeat the argument above and bound the error in the gradient of each $f_i$.


